Arrangements of Submanifolds and the Tangent Bundle Complement

Drawing parallels with hyperplane arrangements, we develop the theory of arrangements of submanifolds. Given a smooth, finite dimensional, real manifold $X$ we consider a finite collection $\mathcal{A}$ of locally flat, codimension-1 submanifolds that intersect like hyperplanes. To such a collection we associate two combinatorial objects: the face category and the intersection poset. We also associate a topological space to the arrangement called the tangent bundle complement. It is the complement of union of tangent bundles of these submanifolds inside the tangent bundle of the ambient manifold. Our aim is to investigate the relationship between the combinatorics of the arrangement and the topology of the complement. In particular we show that the tangent bundle complement has the homotopy type of a finite cell complex. We generalize the classical theorem of Salvetti for hyperplane arrangements and show that this particular cell complex is completely determined by the face category.

==> content/section5.tex <==
\section{Homotopy Theory of the Tangent Bundle Complement} \label{sec:CoversOfTheSalvettiComplex}

 
In this section we focus on the homotopy theory of the tangent bundle complement. We start by defining the arrangement groupoid. This is a generalization of the groupoid \emph{Gal} introduced by Deligne in \cite{deli72} and also of the oriented systems introduced by Paris in \cite{pa1}. We then look at the covering spaces of the Salvetti complex, our aim is to show that they are also determined combinatorially. We prove this by generalizing the theory of \emph{Salvetti-type diagram models} introduced by Delucchi in \cite{del1} (building on the work of Paris \cite{pa1}) to submanifold arrangements. The classification of the covering spaces is done at the end. \par

\subsection{The fundamental group(oid)} \label{sec:TheFundaGroup}
We start by extending the idea of an \emph{arrangement graph}, associated with a hyperplane arrangement (see \cite{del1, deli72, pa1}). 

\bd{def1c3s4}
Given an arrangement of submanifolds $\A$ in a manifold $X$, the arrangement graph, denoted by $G(\A)$, is the oriented $1$-skeleton of the associated Salvetti complex. \ed 

A \emph{path} in the arrangement graph is a sequence of edges traversed not necessarily according to their orientations. The length of a path is equal to the number of edges traversed. An edge is a path of length $1$ and vertex is path of length $0$. Initial vertex of a path $\alpha$ is denoted by $s(\alpha)$ and the terminal vertex by $t(\alpha)$. Such directed paths can be represented by words whose letters correspond to edges. If $\alpha$ is an undirected path then $\alpha = (\epsilon_1 a_1, \dots, \epsilon_n a_n)$ where $\epsilon_i = \pm 1$ depending on whether $a_i$ is traversed along or opposite to its orientation, the length of $\alpha$ is equal to $n$ and $s(\epsilon_{i+1}a_{i+1}) = t(\epsilon_i a_i)$ for every $i$. If $\alpha$ and $\beta$ are two paths such that $s(\beta) = t(\alpha)$ then their concatenation gives a new path denoted by $\alpha\beta$ (note that this is not a composition of functions). Inverse of a path $\alpha = (\epsilon_1 a_1, \dots, \epsilon_n a_n)$ is the path $\alpha^{-1} = (-\epsilon_n a_n, \dots, -\epsilon_1 a_1)$. \par 

A \emph{directed path} is a sequence of consecutive edges traversed according to their orientations.  For example, $\alpha = (+a_1,\dots, +a_n)$ is a directed path of length $n$. A \emph{minimal positive path} is a path having shortest length among all the positive paths that join its endpoints. Unless otherwise stated by a \emph{path} we mean an \emph{undirected path} and by a \emph{positive path} we mean a directed path.\par

Recall that every $2$-cell in the Salvetti complex is a polygon with an even number of (oriented) edges and that the boundary of such a $2$-cell is composed of two minimal positive paths of same length (Corollary \ref{cor2s3c3}). \par

We define two types of `\emph{moves}' on the paths in the arrangement graph:
\begin{enumerate}
	\item If $\alpha$ is a path such that $\alpha = \alpha_1\gamma\alpha_2$ and if $\gamma, \gamma'$ are two minimal positive paths joining the opposite vertices of a $2$-cell, then substitute $\gamma'$ for $\gamma$ in $\alpha$. 
	\item If $\alpha$ is a path such that $\alpha = \alpha_1\gamma\alpha_2$, where $\gamma$ is a sub-path of a boundary path of a $2$-cell of $Sal(\A)$, substitute for $\gamma$ the path $\gamma'$ having same endpoints (i.e. $s(\gamma') = s(\gamma), t(\gamma') = t(\gamma)$) and containing all the remaining edges of that $2$-cell. 
\end{enumerate}
Note that the above `moves' define a homotopy between the directed paths.
\bd{def2c3s4}
Given a submanifold arrangement $\A$, the associated \emph{category of positive paths}, (positive category for short) denoted by $\G^+(\A)$, is the category of directed paths in the Salvetti complex. \ed 

Recall that (see, for example, \cite[Chapter 3]{pjh} ) the objects of this category are the vertices of the arrangement graph. The morphisms are equivalence classes of positive paths. Two positive paths $\alpha$ and $ \beta$ from a vertex $C$ to a vertex $D$ are equivalent if and only if $\alpha$ is obtained from  $\beta$ by a finite sequence of moves of type $(1)$. It means that the two paths are connected by a sequence of substitutions of minimal positive paths. This equivalence relation will be called the \emph{positive equivalence}, the equivalence class of a path $\alpha$ will be denoted by $[\alpha]_+$ and the relation denoted by $\stackrel{+}{\sim}$. \par

In case of hyperplane arrangements any two minimal positive paths with the same end points are homotopic in the associated Salvetti complex. Hence represent the same morphism in the positive category. However this need not be true for submanifold arrangements. For example, consider the Salvetti complex (Figure \ref{circsal}) associated to the arrangement of $2$ points in $S^1$ (Example \ref{ex41}). The two edges labeled $[p, A]$ and $[q, A]$ are minimal positive paths with the same end points however they are  not positive equivalent. 

\bl{lem1newc3s4}
Let $F$ be a face of a submanifold arrangement and $C$ be a chamber such that $C\prec F$ in $\F^*$. Then any two minimal positive paths from $C$ to $F\ast C$ are positive equivalent. \el

\bpr 
The statement follows from the application of Corollary \ref{cor2s3c3}. Any two minimal positive paths from $C$ to $F\ast C$ are in fact contained in the boundary of the cell $[F, C]$. \epr 

Hence we can rephrase the positive equivalence as follows. Let $\alpha, \alpha'$ be two positive paths from $C$ to $C'$. Set $\alpha \stackrel{+}{\sim} \alpha'$ if and only if $\alpha = \alpha_1\beta\alpha_2$, $\alpha' = \alpha_1\beta'\alpha_2$ such that 
\begin{enumerate}
	\item $\alpha_1$ is a positive path from $C$ to $C''$,
	\item $\beta$ and $\beta'$ are minimal positive paths from $C''$ to $F\ast C''$ (for some $C''\prec C$),
	\item $\alpha_2$ is a positive path from $F\ast C''$ to $C'$.
\end{enumerate}
%More generally, set $\alpha \stackrel{+}{\sim}\alpha'$ if and only if $\alpha$ is obtained from $\alpha'$ by a finite sequence of positive paths related as above. We now define the arrangement groupoid.

\bd{def3c3s4}
The \emph{arrangement groupoid} of a submanifold arrangement is a category whose objects are the vertices of the arrangement graph. The morphisms in this category are equivalence classes of paths. Two paths are equivalent if and only if one is obtained from the other by a finite sequence of moves of type $(2)$. The category will be denoted by $\G(\A)$ and the morphisms will be denoted by $[\alpha]$, where $\alpha$ is a representative path. \ed

The reader familier with homotopy theory will realize that the arrangement groupoid is the free groupoid on the Salvetti poset (consequently the fundamental groupoid of its nerve, the Salvetti complex). We state this as a result.

\bl{lem2c3s4} Let $\A$ be an arrangement of submanifolds in a manifold $X$. The arrangement groupoid $\G(\A)$ is equivalent to the fundamental groupoid $\fgp(Sal(\A))$ of the associated Salvetti complex. \el

 Before moving on we would like to explicitly state the relationship between the above defined categories. 

\bt{thm1c3s4} For a submanifold arrangement $\A$ the category $\G(\A)$ can be identified with the category of fractions of $\G^+(\A)$ and the associated canonical functor $J\colon \G^+ \to \G $ is defined by sending $[\alpha]_+$ to $[\alpha]$. \et

\bpr The proof follows from the observation that the moves of type $(2)$ are composed of moves of type $(1)$ and the definition of category of fractions (see \cite[Chapter 1]{gabzis67}). \epr

By studying the $2$-skeleton of $Sal(\A)$ we can deduce a presentation for the fundamental group. 

\bt{thm2s5c3}
Let $X$ be a $l$-manifold and $\A$ be an arrangement of submanifolds with $Sal(\A)$ being the associated Salvetti complex. If $X$ is simply connected then two minimal positive paths in the $1$-skeleton of $Sal(\A)$ that have same initial as well as terminal vertex are homotopic. \et 

\bpr
Let $\alpha, \beta$ be two positive paths such that $s(\alpha) = s(\beta) =[C, C]$, $t(\alpha) = t(\beta) = [D, D]$ and both of them have same lengths ($= d(C, D)$). Clearly, $\psi(\alpha), \psi(\beta) \subset X^*_1$ (recall that $\psi\colon Sal(\A)\to X^*$ was defined in Theorem \ref{thm2s3c3}) are minimal paths of length $d(C, D)$, so no two edges of these two paths are sent (by $\psi$) to the same edge of $X^*$. Without loss of generality, let $a = [F^1, C']$ be an edge of the path $\alpha$, consider $(a)$ as a sub-path of $\alpha$. Let $s(a) = [C', C']$ then, $F^1\circ C = C'$ since $\alpha$ is minimal. Repeating same argument for every edge of $\beta$ we get that the paths $\alpha$ and $\beta$ are contained in $\iota_C(X^*)$. Hence by Theorem \ref{thm2s3c3} and the fact that $\pi_1(X^*) = \{ 1\}$, it follows that $\alpha$ and $\beta$ are homotopic. \epr

An immediate consequence of this theorem is the following:

\bc{cor1s5c3}
If $X$ is a $l$-manifold, $\A$ is an arrangement of submanifolds and $M(\A)$ is the tangent bundle complement then,
\[\pi_1(M(\A)) \cong \pi_1(G(\A)) / \{\alpha \beta^{-1} ~|~ \alpha, \beta \hbox{~ are minimal positive paths with same end points}\}.\] \ec

\bpr A loop in the arrangement graph $G(\A)$ is contractible if and only if it is the boundary of a $2$-cell (of $Sal(\A)$). According to Corollary \ref{cor2s3c3} the boundary of every $2$-cell is composed of two minimal positive paths with same ends. \epr

In particular Theorem \ref{thm2s5c3} applies to hyperplane arrangements and arrangements in a sphere (dimension $\geq 2$). Minimal positive paths with same end points are homotopic in the Salvetti complex. Hence these paths represent the same morphism in the corresponding arrangement groupoid. More is true for (central) hyperplane arrangements; minimal positive paths with same end points represent same morphism in the positive category (see \cite[1.12]{deli72} for the original proof). This means that the restriction of functor $J$ to the class of minimal positive paths is faithful (this holds true even for arrangements of pseudospheres \cite[Theorem 20]{salvetti93} and pseudohyperplanes \cite[Chapter 5]{deshpande_thesis11}).

\bl{lem1s6c3}
Let $\A$ be an arrangement of submanifolds in a $l$-manifold $X$.
If $\pi_n(X) \neq 0$ then $\pi_n(M(\A)) \neq 0$. \el

\bpr
Follows from Theorem \ref{thm37}. \epr

The only hope to find $K(\pi, 1)$ complements is to consider arrangements in $K(\pi, 1)$ manifolds.

\subsection{Salvetti-type diagram models}\label{sec:stdm}

The covering spaces of a topological space can be classified by their fundamental groupoids. According to \cite[Chapter 10]{brn1}, the connected covers of the fundamental groupoid correspond to fundamental groupoids of the corresponding covering spaces (see also \cite[Chapter 13]{pjh}). The fundamental group of the Salvetti complex is isomorphic to the object group $\pi(\G)$. Hence the connected topological covers of the Salvetti complex are indexed by the subgroups of $\pi(\G)$ (and so are the groupoid covers of $\G(\A)$). We will use this correspondence to first, construct the covering spaces of $Sal(\A)$  and then, to classify them.\par 

The use of this idea can be traced back to the work of Deligne in \cite{deli72}, where he used this correspondence to construct the universal cover of the hyperplane complement. Then Paris generalized these arguments, using the language of oriented systems (see \cite{pa1}), to show that all of the connected covers of any arrangement complement are indexed by the covers of the arrangement groupoid. Our treatment here is based on Delucchi's reformulation \cite{del1, del07} of these ideas in terms of diagram of spaces. 
To be precise, using covers of the arrangement groupoid he defined a family of diagrams of spaces such that their homotopy colimits have the homotopy type of covers of arrangement complement. One of the benefits of his elegant treatment is that it is easy to generalize to the tangent bundle complement. This is what we plan to do now. We closely follow Delucchi's arguments as well as the notation.\par

Let $\A$ denote a submanifold arrangement in some manifold $X$. Let $Sal(\A)$ be the associated Salvetti complex, the context will decide whether we view it as a CW-complex or as simplicial complex. Finally, let $\G$ denote the arrangement groupoid. When dealing with morphisms in $\G$ we will use the path-terminology. For example, domain of a morphism $[\alpha]$ will be denoted by $s(\alpha)$. Hence whenever we make statement about a path it is actually about its equivalence class in $\G$. \par

For the convenience of the reader we quickly recall relevant facts about the cover of a groupoid. Given $z \in Ob(\G)$ its \emph{star} is the following set of morphisms-
\[St(z) = \{[\alpha]\in Mor(\G)~|~ s(\alpha) = z\}. \] 
A \emph{covering} of $\G$ is a functor $\rho\colon \G_{\rho}\to \G$ such that for every $z\in Ob(\G_{\rho})$, the induced map 
\[\rho_z\colon St(z) \to St(\rho(z)) \]
is bijective. Given $[\alpha]$, a morphism in $\G$ and any $z\in \rho^{-1}(s(\alpha))$, the lift of $\alpha$ at $z$ is the morphism $\rho^{-1}_z(\alpha)$, denoted by $\alpha^{<z>}$ when the covering $\rho$ is understood. Recall that according to the main theorem of \cite[Chapter 10]{brn1} each object of $\G_{\rho}$ is a right coset of homotopy class of paths in the arrangement graph. Let $\mu(C\to D, F)$ denote a minimal positive path starting at a vertex $[C, C]$ ending at another vertex $[D, D]$ and it traverses an edge contained in the boundary of $[F, C]$. It is assumed that $C\prec F$. 


\bl{lem3c3s4} With the same notation as above, $\mu(C\to D, F)\stackrel{+}{\sim} \mu(C\to D, F')$ if there exists $G\in \F^*$ such that one of the following is satisfied:
\begin{enumerate}
	\item $F, F'\prec G$ and $\mu(C\to D, F), \mu(C\to D, G)$ are in the boundary of $[G, C]$;
	\item $D = G\ast C$.
\end{enumerate} \el
 
\bpr Follows from Corollary \ref{cor2s3c3}. \epr 


\bd{def1s4c3}
Given a cover of the arrangement groupoid $\rho\colon\G_{\rho}\to\G(\A)$, we define a \emph{diagram of posets} $\D_{\rho}$ on the dual face poset $\F^*$ as 
\[\D_{\rho}(F^i) := \{ v\in Ob(\G_{\rho}) ~|~ \rho(v) \prec F^i\}. \]
Each poset is endowed with the trivial order relation. The maps between these spaces are the following inclusions
\beq
 \D_{\rho}(F^i\to F^j)\colon \D(F^i)&\to& \D(F^j) \quad (i > j)\nn \\
 											 v &\mapsto& t(\mu(\rho(v)\to F^j\circ \rho(v), F^i)^{<v>}) \nn
\eeq 
where $\mu(\rho(v)\to F^j\circ \rho(v), F^i)^{<v>}$ is the lift of the minimal positive path in $\G$ that starts at $[\rho(v), \rho(v)]$ and traverses an edge contained in $[F^i, \rho(v)]$. \ed

According to the \emph{simplicial model lemma} (Lemma \ref{lem35}), the homotopy colimit of the above diagram is in fact an order complex. We will denote this order complex by $\s_{\rho}$, its vertex set is 

\[ \{(F, v)\in \F^*\times Ob(\G_{\rho}) ~|~ \rho(v) \prec F \} \]

the simplices of $\s_{\rho}$ are chains with respect to the following partial order
\[(F_2, v_2)\prec_{\rho} (F_1, v_1)\Leftrightarrow \begin{cases}F_2\prec F_1\hbox{~and}\\ 
v_2 = t(\mu(\rho(v_1)\to F_2\circ \rho(v_1), F^1)^{<v_1>}) \end{cases} \]

\br{rem1s4c3} If $\rho$ is the identity map then $\s_{id}$ is the Salvetti complex (Theorem \ref{thm5s3c3}).\er

\br{rem2s4c3}
Using the same arguments as in the proof of Lemma \ref{lem350} it follows that for every chain in $\s_{\rho}$ there corresponds a chain and a vertex in $\F^*$. If $\phi$ is a chain in $\F^*$ and $v\in Ob(\G_{\rho})$ such that $\rho(v) \prec max(\phi)$, then the pair $(\phi, v)$ corresponds to a chain in $\s_{\rho}$ and every chain is of this form. Moreover, the simplicial complex $\Delta(\s_{\rho})$ is the barycentric subdivision of a CW-complex $\s_{\rho}^{CW}$; the barycentric subdivision of a (closed) $k$-cell of this CW-complex, which we denote by a pair $[F^k, v]$, is given by 
\[ [F^k, v] := \bigcup_{max(\phi) = F^k} (\phi, v).\]
Vertices of $\s_{\rho}^{CW}$ are of the form $[\rho(v), v]$, hence are in bijection with the objects of $\G_{\rho}$. For a $k$-cell $[F^k, v]$ a $0$-cell $[\rho(v'), v']$ is its vertex if and only if 
$$v' = t(\mu(\rho(v)\to F'\circ \rho(v'), F^k)^{<v>})$$ 
for some $F'\prec F^k$. \er

Our aim is to show that the simplicial complex $\s_{\rho}$ is a covering space of the (simplicial) Salvetti complex. The strategy we employ here is motivated by the proof of a well known fact in elementary algebraic topology. A simplicial and fixed point free action of a discrete group on a simplicial complex is a covering space action (see for example \cite[Section 1.B]{hatcher02}). First, we prove that there is a natural, simplicial map between these two complexes and then proceed on to prove that it is indeed a covering map.\par

The functor $\rho\colon\G_{\rho}\to\G$ naturally induces a morphism of diagrams $\lambda\colon\D_{\rho}\to \D_{id}$. On the level of spaces it is given by:
\begin{eqnarray*}
\lambda_{F}\colon  \D_{\rho}(F)&\to& \D_{id}(F) \quad \forall F\in \F^* \\
									 v &\mapsto& \rho(v).  \end{eqnarray*}
In order to check the compatibility of this morphism with the maps between the spaces, consider $F_2\prec F_1$ and $v\in \D_{\rho}(F_2)$. Then,
\begin{eqnarray*} 
\lambda_{F_2}(\D_{\rho}(F_1\to F_2)(v)) &=& \rho(t(\mu(\rho(v)\to F_2\circ \rho(v), F_1)^{<v>})) \nn\\
																				&=& F_2\circ \rho(v) \nn \\	
																				&=& \D_{id}(F_1\to F_2)(\rho(v)) \nn \\
																				&=& \D_{id}(F_1\to F_2)(\lambda_{F_1}(v)).\nn
\end{eqnarray*}
The morphism $\lambda$ induces a map between homotopy colimits by functoriality, hence a map of simplicial complexes 
\[\Lambda_{\rho}\colon \s_{\rho} \to Sal(\A). \]
$\Lambda_{\rho}$ maps the simplex $(\phi, v)$ of $\s_{\rho}$ to the simplex $(\phi, \rho(v))$ of $Sal(\A)$. Moreover, a morphism $\eta\colon\G_{\rho_1}\to\G_{\rho_2}$ between two covers of the arrangement groupoids induces a map $\Lambda_{\eta}\colon \s_{\rho_1}\to \s_{\rho_2}$. 

\bt{thm1s4c3}
The map $\Lambda_{\rho}\colon\s_{\rho}\to Sal(\A)$, induced by a cover $\rho\colon\G_{\rho}\to\G$ of the arrangement groupoid, is a covering map. \et

\bpr
First note that $Sal(\A)$ is a finite dimensional and locally finite simplicial complex implying that it is connected and locally path connected. Hence all its connected covering spaces exist. \par
Let $p\in Sal(\A)$ be some point, $\sigma$ be the smallest dimensional simplex containing $p$, let $U$ denote the star of $\sigma$ (set of all simplices of $Sal(\A)$ that contain $\sigma$). In order to show that $\Lambda_{\rho}$ is a covering map it is enough to show that $\Lambda_{\rho}^{-1}(U)$ is an even covering of $U$. \par

Let us first characterize $U$ and its inverse image in terms of chains and chambers. As $\sigma$ is a simplex of $Sal(\A)$ there exists a chain $\tilde{\phi}$ in $\F^*$ and (a chamber) $\tilde{C}\prec max(\tilde{\phi}) =: \tilde{F}$ such that $\sigma = (\tilde{\phi}, \tilde{C})$. Thus star of $\sigma$ takes the following form:
\[U = \bigcup_{\substack{\phi\supseteq\tilde{\phi}\\ C\in R(\phi,\tilde{C})}} (\phi, C) \]
where $R(\phi, \tilde{C}) := \{C \prec max(\phi)~|~ \tilde{F}\circ C= \tilde{C} \}$. 
As a set, the pre-image of $U$ is:
\[\Lambda_{\rho}^{-1}(U) = \bigcup_{\substack{\phi\supseteq\tilde{\phi} \\ \{v ~|~ \rho(v)\in R(\phi,\tilde{C})\}}} (\phi, v). \]
\noindent For a fixed object $w\in \rho^{-1}(\tilde{C})$ define
\[W_{w} := \bigcup_{\substack{\phi\supseteq\tilde{\phi} \\ C\in R(\phi,\tilde{C})}}(\phi, v(C, w)) \]
where $v(C, w)$ is the (unique) object, of $\G_{\rho}$, in $\rho^{-1}(C)$ from which $w$ can be reached by the lift of a minimal positive path. \par

Rest of the proof follows from the following three claims which are left as an exercise. \par

\textbf{Claim 1:} For any $w_1\neq w_2 \in \rho^{-1}(\tilde{C}), ~W_{w_1}\cap W_{w_2} = \emptyset$.\par
%Assume that the intersection is non-empty and there is a simplex $$(F, u)\subset W_{w_1}\cap W_{w_2}.$$ 
%By definition of $W_w$,
%\[u = v(C, w_1) = v(C, w_2) \]
%and $\rho(u) = C$. This is same as 
%\begin{eqnarray*}
%w_1 &=& t(\mu(C\to \rho(w_1), F)^{<u>})  \\
%w_2 &=& t(\mu(C\to \rho(w_2), F)^{<u>}) \end{eqnarray*}
%which implies $w_1 = w_2$ (since $\rho(w_1) = \rho(w_2) = \tilde{C}$), a contradiction. \par

\textbf{Claim 2:} \[\coprod_{w\in \rho^{-1}(\tilde{C})}W_{w} = \Lambda_{\rho}^{-1}(U). \]
%To see that the left hand side is contained in the right hand side, consider a simplex $(\phi, v(C, w))$. Its image $\Lambda_{\rho}(\phi, v(C, w)) = (\phi, C)$ is a simplex of the right hand side. \par

%For the converse, consider $(\phi, v)$ a simplex of the left hand side (such that $\tilde{\phi}\subseteq \phi$ and $\rho(v)\in R(\phi, \tilde{C})$). Define $w := t(\mu(\rho(c)\to \tilde{C}, max(\phi))^{<v>})$. By construction, $\rho(w) = \tilde{C}$, hence $(\phi, v)$ is a simplex of $W_w$.\par

\textbf{Claim 3:} Fix $w\in \rho^{-1}(\tilde{C})$, then $\Lambda_{\rho}\colon W_w\to U$ is a homeomorphism.\epr
%Clearly $\Lambda_{\rho}$ is a simplicial map and also it is surjective, since given $(\phi, C)$ a simplex of $U$, $(\phi, v(C, w))$ is a simplex of $W_w$ which lies in its pre-image. The injectivity of this map follows from \cite[Lemma 4.3.3]{del1} and \cite[Lemma 3]{sal1}. \epr

\be{ex1s4c3}
Consider the arrangement $\A_1$ of $2$ points in $S^1$ (Example \ref{ex41}), its associated Salvetti complex $Sal(\A_1)$ was described in Figure \ref{circsal}. Figure \ref{covercirc} depicts a portion of its universal cover. The objects of the covering groupoid are denoted by $\tilde{A}, \tilde{B}$ (indices are suppressed for notational simplicity). 
\begin{figure}[!ht]
\begin{center}
	\includegraphics[scale=0.51,clip]{img/covercirc.pdf}
\end{center}\caption{The Universal cover of $Sal(\A_1)$}\label{covercirc} 
\end{figure} 
Note that there are two minimal positive paths, in $Sal(\A)$, from $[B, B]$ to $[A, A]$. One of them is the (oriented) edge $[p, B]$ and the other is the edge $[q, B]$. Both of these paths are represent distinct equivalence classes in $\G^+(A)$ as well as $\G(A)$. In the covering space, end points of the lifts of these two paths are distinct and are contained in $\rho^{-1}([A, A])$. Also note that the functor $J\colon \G^+(A)\to \G(A)$ is faithful in this example. \ee

Now we prove that any connected topological covering space of the Salvetti complex corresponds to a Salvetti-type diagram model. We use the correspondence between isomorphism classes of covering spaces and conjugacy classes of subgroups (\cite[Theorem 1.38]{hatcher02}). \par

Given a cover $\rho\colon \G_{\rho}\to \G$ of the arrangement groupoid $\G$, consider the corresponding covering cell complex $\s_{\rho}$ of the associated Salvetti complex $Sal(\A)$ (see Remark \ref{rem2s4c3}). \par

\noindent\textbf{$2$-skeleton}: For a codimension $2$ face $F^2$ and an object $v\in Ob(\G_{\rho})$ (such that $\rho(v)\prec F^2$) there is one $2$-cell $[F^2, v]$ in $\s_{\rho}$. The vertices of $[F^2, v]$ are indexed by the chambers whose closures contain $F^2$. To such a chamber $C$, there corresponds an object in the covering groupoid given by $t(\rho(v)\to C, F^2)^{<v>}$. Hence the vertex set of $[F^2, v]$ is given by $\{[\rho(v_i), v_i] ~|~ \rho(v_i)\prec F^2, i = 1,\dots, 2k \}$. A $1$-cell $[F^1, v_i]$ in the boundary of $[F^2, v]$ corresponds to codimension $1$ face $F^1$ such that $F^1\prec F^2$. The vertex $v_1$ is such that the chamber $\rho(v_i)$ is on the same side as $\rho(v)$ with respect to $F^1$. Moreover, the cell is oriented to have $v_i$ as its start vertex. \par

\br{rem4c3s5}
Attachment of higher dimensional cells is analogous to the construction of Salvetti complex. Hence it can be shown that these covering complexes $\s_{\rho}$ have the structure of a MH-complex.\er

The next step in the classification is to show that the fundamental group of $\s_{\rho}$ is isomorphic to the object group of $\G_{\rho}$. We compare the relations given by $2$-cells of $\s_{\rho}$ and the relations that define $\G_{\rho}$. \par

Recall that the equivalence relation in the arrangement groupoid $\G$ is generated by identifying two paths with same end points which form the boundary of a $2$-cell in $Sal(\A)$. As a result, the identity in an object group is an equivalence class of loops based at that object that can be written as $\gamma \gamma'^{-1}$, where $\gamma, \gamma'$ are paths bounding a $2$-cell. For a given groupoid cover $\rho\colon\G_{\rho}\to \G$ let $G_{\rho}$ denote the graph underlying $\G_{\rho}$. The morphisms of $\G_{\rho}$ are equivalence classes of paths in the graph $G_{\rho}$. This equivalence relation is the one induced by $\rho$. To be precise, two paths $\tilde{\alpha}, \tilde{\beta}$ in $G_{\rho}$ are identified if and only if they have same end points and $\rho(\tilde{\alpha}) \sim \rho(\tilde{\beta})$ (where $\tilde{\alpha}, \tilde{\beta}$ are lifts of $\alpha, \beta$ respectively). Hence the relations in $\G_{\rho}$ are generated by the loops of the form $\tilde{\gamma_1}\tilde{\gamma_2}^{-1}$ such that $[\gamma_1] = [\gamma_2]$ (in $\G_{\rho}$), denote the normal subgroup generated by these loops by $\Sigma_{\rho}$. In a nutshell we have $\pi(\G_{\rho}) \cong \pi_1(G_{\rho}) / \Sigma_\rho$.\par

On the other hand let $\sigma_{\rho}$ denote the smallest normal subgroup of $\pi_1((\s_{\rho})_1)$ generated by the relations imposed by the boundary of every $2$-cell. Then, $\pi_1(\s_{\rho}) \cong \pi_1((\s_{\rho})_1) / \sigma_{\rho}$. 


\bt{thm4s5c3} With the notation as above: $$\pi(\G_{\rho}) \cong \pi_1(\s_{\rho}).$$  \et

Now we are in the position to state the classification of covering spaces of the Salvetti complex. 
\bt{thm5s5c3}
Let $\A$ be a submanifold arrangement in a $l$-manifold $X$, let $Sal(\A)$ denote the associated Salvetti complex and $\G$ denote the arrangement groupoid. For any topological cover $p\colon S\to Sal(\A)$, there exists a cover of the arrangement groupoid $\rho\colon\G_{\rho}\to\G$ such that the homotopy colimit of the associated diagram of spaces $\D_{\rho}$ is isomorphic to $S$ as a covering space of $Sal(\A)$ \et

\bpr
Let $H$ denote the isomorphic image of $p_*(\pi_1(S))$ inside $\pi(\G(\A))$ (under the isomorphism in Theorem \ref{thm4s5c3}). As a result of \cite[Theorem 10.6.1]{brn1} we see that there is a covering groupoid $\rho\colon \G_{\rho}\to \G(A)$ such that $\pi(\G_{\rho})\cong H$. Let $S_{\rho}$ denote the homotopy colimit of the diagram of spaces defined using $\G_{\rho}$. Again appealing to Theorem \ref{thm4s5c3} it implies that $\pi_1(S_{\rho}) \cong H$. Let $\iota_{\rho}$ denote the inclusion of $G_{\rho}$ (the graph underlying $\G_{\rho}$) into $S_{\rho}$ as its $1$-skeleton. Since $\G_{\rho}$ is equivalent to the fundamental groupoid of $S_{\rho}$ the following diagram commutes. 
  \[ 
  \begin{CD}
  \pi(\G_{\rho}) @>\cong >> \pi_1(S_{\rho})\\
    @V\rho_* VV @VV(\Lambda_{\rho})_* V \\
    \pi(\G) @>{\cong}>> \pi_1(Sal(\A)) \\
  \end{CD}
  \]
Since $(\Lambda_{\rho})_*(S_{\rho})\cong H$ we have that $S$ and $S_{\rho}$ are isomorphic as covering spaces. \epr

\bc{cor3s5c3}
Any cover $p\colon S\to Sal(\A)$ of the Salvetti complex can be realized as the order complex of a poset. \ec

\bc{cor4s5c3}
Let $\hat{\rho}\colon\G_{\hat{\rho}}\to\G$ denote the universal cover of the arrangement groupoid. Then $\s_{\hat{\rho}}$, the homotopy colimit of the associated diagram of spaces (posets) is the universal cover of $Sal(\A)$. \ec




